Supporting mixed-datatype matrix multiplication within the BLIS framework

We approach the problem of implementing mixed-datatype support within the general matrix multiplication (GEMM) operation of the BLIS framework, whereby each matrix operand A, B, and C may be stored as single- or double-precision real or complex values. Another factor of complexity, whereby the computation is allowed to take place in a precision different from the storage precisions of either A or B, is also included in the discussion. We first break the problem into mostly orthogonal dimensions, considering the mixing of domains separately from mixing precisions. Support for all combinations of matrix operands stored in either the real or complex domain is mapped out by enumerating the cases and describing an implementation approach for each. Supporting all combinations of storage and computation precisions is handled by typecasting the matrices at key stages of the computation---during packing and/or accumulation, as needed. Several optional optimizations are also documented. Performance results gathered on a 56-core Marvell ThunderX2 and a 52-core Intel Xeon Platinum demonstrate that high performance is mostly preserved, with modest slowdowns incurred from unavoidable typecast instructions. The mixed-datatype implementation confirms that combinatoric intractability is avoided, with the framework relying on only two assembly microkernels to implement 128 datatype combinations.

==> abstract.tex <==
Matrix-matrix multiplication is a computation of fundamental importance in  scientific computing.  The Basic Linear Algebra Subroutines (BLAS) interface supports a large number of cases of $ C := \alpha \op( A) \op(B) + \beta C $: while all three matrices are stored with column-major order, the matrices can {\em all} be of different precision (single or double precision floating point) and type (real or complex), and $ \op $ can be ``No transpose, ``transpose,'' or ''Conjugate transpose.''  This requires an implementation to  support $ 2 \times 2 \times 2^3 = 32 $ cases.  In practice, each matrix can be of a different precision or type, $ \op $ can also be conjugation without transposition, and each of the matrices may be stored in column-major order, row-major order, or with general row and column stride.  To accommodate this, the number of case grows to $ 2^3 \times 2^3 \times 4^2 \times 3^3  = 9216 $.
Some applications in scientific computing now require use of extended precision while for applications in Machine Learning sometimes half precision (16 bit)suffices.
 This paper discusses a high-performance implementation that manages the resulting complexity, focusing on the subproblem when the precision is identical for all three matrices, but the type (real or complex) can be different.  This means ??? cases must be handled.
